Non-stationary Bandits and Meta-Learning with a Small Set of Optimal Arms

We study a sequential decision problem where the learner faces a sequence of $K$-armed bandit tasks. The task boundaries might be known (the bandit meta-learning setting), or unknown (the non-stationary bandit setting). For a given integer $M\le K$, the learner aims to compete with the best subset of arms of size $M$. We design an algorithm based on a reduction to bandit submodular maximization, and show that, for $T$ rounds comprised of $N$ tasks, in the regime of large number of tasks and small number of optimal arms $M$, its regret in both settings is smaller than the simple baseline of $\tilde{O}(\sqrt{KNT})$ that can be obtained by using standard algorithms designed for non-stationary bandit problems. For the bandit meta-learning problem with fixed task length $\tau$, we show that the regret of the algorithm is bounded as $\tilde{O}(NM\sqrt{M \tau}+N^{2/3}M\tau)$. Under additional assumptions on the identifiability of the optimal arms in each task, we show a bandit meta-learning algorithm with an improved $\tilde{O}(N\sqrt{M \tau}+N^{1/2}\sqrt{M K \tau})$ regret.

==> m small 10-18-2022_arXiv/body.tex <==






\begin{abstract}
  We study a sequential decision problem where the learner faces a sequence of $K$-armed bandit tasks. %
  The task boundaries might be known (the bandit meta-learning setting), or unknown (the non-stationary bandit setting). For a given integer $M\le K$, the learner aims to compete with the best subset of arms of size $M$.  
  We design an algorithm based on a reduction to bandit submodular maximization, and show that, for $T$ rounds comprised of $N$ tasks, in the regime of large number of tasks and small number of optimal arms $M$, its regret in both settings is smaller than the simple baseline of $\tilde{O}(\sqrt{KNT})$ that can be obtained by using standard algorithms designed for non-stationary bandit problems. For the bandit meta-learning problem with fixed task length $\tau$, we show that the regret of the algorithm is bounded as $\tilde{O}(NM\sqrt{M \tau}+N^{2/3}M\tau)$. Under additional assumptions on the identifiability of the optimal arms in each task, we show a bandit meta-learning algorithm with an improved $\tilde{O}(N\sqrt{M \tau}+N^{1/2}\sqrt{M K \tau})$ regret.
\end{abstract}

\section{Introduction}


Consider a recommendation platform with a large catalog of items. 
Every day, the system gets to interact with different customers and must sequentially discover what is the preferred item of the day. But if we suppose that days correspond to recurring groups of customers, it naturally implies that only a small subset of the catalog is eventually preferred.
In this problem, like in many personalization or recommendation scenarios, the learner needs to solve a sequence of tasks.
When the tasks share some similarities, the learner may be able to utilize this by sequentially learning the underlying common structure in the tasks and hence perform better on the sequence than solving each task in isolation. In this paper we study a special class of these \emph{meta-learning} problems, where each task is an instance of a multi-armed bandit problem.

Formally, we consider a problem where a learner faces $N$ instances of $K$-armed bandit tasks sequentially. At the beginning of task $n\in [N]$,\footnote{For any integer $k$, we let $[k]=\{1,2,\dots,k\}$, and for any (multi-)set $S$, $|S|$ denotes the number of distinct elements in $S$.} the adversary  chooses the mean reward function $r_{n}\in \cR=[0,1]^K$. 
Then, the learner interacts with the $K$-armed bandit task specified by the reward function $r_n$ for $\tau_n$ time steps: for each $n\in [N]$, when action $a \in [K]$ is played, it receives reward $r_n(a)+\eta_{n,t}(a)$ where $\eta_{n,t}(a)$ are independent zero-mean and $[-1/2,1/2]$-valued noise variables for all $n,t$ and $a$, so that the expected reward is $r_n(a)$.

We consider two settings: the \emph{meta-learning setting} where the learner knows the length $\tau_n$ of each task $n$ when it starts, and the more general \emph{non-stationary setting} where the task boundaries are unknown~\citep{WL-2021,HKZCAGB-2020,Russac-Vernade-Cappe-2019,Auer-2019}. 


We use $T$ to denote the total number of rounds, $T=\sum_{n=1}^N \tau_n$. Let $\cH_{n,t}$ be the history of the learner's actions and the corresponding observed rewards up to, but not including, time step $t$ in task $n$. For this time step, the learner chooses a distribution $\pi_{n,t}$ over the actions as a function of $\cH_{n,t}$ and other problem data (such as $T$, and $\tau_n$ in bandit meta-learning), and samples an action $A_{n,t}$ from $\pi_{n,t}$ to be used in this time step. The learner's policy $\pi$ is a collection of the mappings $\pi_{n,t}$ (formally, $\pi$ is a mapping from the set of possible histories to distributions over the action set $[K]$). Its regret on a sequence of reward functions $(r_n)_{n=1}^N$ with respect to a sequence of actions $(a_n)_{n=1}^N$ is defined as
\begin{align*}
R (\pi,T, (r_n)_{n=1}^N, (a_n)_{n=1}^N) = 
\E\left[\sum_{n=1}^N \sum_{t=1}^{\tau_n} r_{n}(a_n) - \sum_{n=1}^N \sum_{t=1}^{\tau_n} r_{n}(A_{n,t}) \right] \,,
\end{align*}
where the expectation is over the random actions of the learner, which may depend on the realization of the noise in the rewards as well as some internal randomness used by the learner. Note that, in the notation, we suppressed the dependence of the regret on the segment lengths $(\tau_n)_{n=1}^N$ and only indicated their sum $T=\sum_{n=1}^N \tau_n$.
The learner's worst-case expected regret relative to the best set of $M$ arms (in the sense of achieving the highest expected reward) is defined as
\begin{align*}
    R_T \doteq R (\pi,T, N,M)
    \doteq \sup_{(r_n)_{n=1}^N}  \max_{\substack{(a_n)_{n=1}^N
    : |\{a_n\}_{n=1}^N|\le M}} R(\pi, T, (r_n)_{n=1}^N, (a_n)_{n=1}^N) \;.
\end{align*}
Note that, as usual in bandit problems, we use the mean reward functions $r_n$ in the regret definition rather than the noisy rewards.
Importantly, the learner competes with a sequence of arms that has at most $M$ distinct elements. We call such problems \emph{sparse} non-stationary bandit problems \citep{Kwon-Perchet-Vernade-2017}. We say a sequence of reward functions $r_{1},\dots,r_{N}$ is \emph{realizable} if there exists a set of arms of size at most $M \le K$ which contains an optimal arm (achieving reward $\max_a r_n(a)$) for every task $n$. Otherwise, the problem is called agnostic. All our results, apart from those in Section~\ref{sec:greedy}, hold in the agnostic setting. In the meta-learning problems, our regret guarantees in fact hold even in the more general adversarial setting where the reward vector can change within each task and regret is defined as 
\begin{align*}
R_T = \sup_{(r_{n,t})_{n=1,t=1}^{N,\tau_n}}  \max_{\substack{(a_n)_{n=1}^N : |\{a_n\}_{n=1}^N|\le M}}\E\left[\sum_{n=1}^N \sum_{t=1}^{\tau_n} r_{n,t}(a_n) - \sum_{n=1}^N \sum_{t=1}^{\tau_n} r_{n,t}(A_{n,t}) \right] \;.
\end{align*}

Our goal in this paper is to provide algorithms achieving small worst-case expected regret for both the above problems. In the bandit meta-learning problem, the task lengths (and therefore, the change points) are known at the beginning of each task, while in the sparse non-stationary bandit problems, the start and duration of tasks are unknown, but the number of tasks $N$ is known at the beginning of the game. 

\subsection{Approach: reduction to bandit subset selection}
\label{sec:approach}

Our approach is based on a reduction to the bandit subset selection problem. We describe it first in the simpler bandit meta-learning problem. A natural solution to this problem is to use an appropriate base bandit algorithm
restricted to the optimal subset of $M$ arms at the beginning of each task. Unfortunately, this set is unknown. Nevertheless, it can be learned, and if the learner identifies the correct subset, a restricted version of the base bandit algorithm can be applied to the next task. For any $K$, let $B_{\tau,K}$ be a worst-case regret upper bound in $\tau$ steps for the \textit{base} $K$-armed bandit algorithm. 
Note that $B_{\tau_n,K}=\widetilde O(\sqrt{K \tau_n})$ for the standard bandit algorithms (such as \UCB and Thompson sampling in stochastic tasks, or EXP3 in adversarial tasks, see, e.g., \citealp{LS-2020}
)
;\footnote{The notation $\widetilde O$ hides polylogarithmic terms.}  accordingly, we assume throughout that $B_{\tau,K}$ is a non-decreasing concave function of both $\tau$ and $K$. When restricted to the correct $M$-subset (i.e, a subset of size $M$ containing the best arm) of the $K$ arms, the regret of the base algorithm is bounded by  $B_{\tau_n,M}\leq B_{\tau_n,K}$.
Otherwise, if the chosen subset does not contain the best arm, the regret on this task can be linear in $\tau_n$. Therefore, it is important to identify the correct subset quickly.

This way the bandit meta-learning problem can be reduced to a bandit subset-selection problem, where the decision space is the set of $M$-subsets of $[K]$ and the reward in round $n$ is the maximum cumulative reward in task $n$ over the chosen subset. For example, when all tasks have length $\tau$, and $\tau\ll N$, an $o(N)$-regret for the bandit subset-selection problem translates to an $O(N B_{\tau,M}) + o(N)$ bound on $R(\pi,T,N,M)$ for the bandit meta-learning problem. Notice that the leading term in the regret is $O(N B_{\tau,M})$, which is an upper bound on the regret of a bandit strategy that runs the base algorithm on the correct subset in each task. The subset-selection problem is a bandit submodular maximization problem, for which the online greedy approximation (\OGO) algorithm\footnote{The superscript $^o$ stands for "opaque" feedback model in the cited paper.}of \citet{streeter2007online} achieves regret $O(N^{2/3})$. 

The approach to the sparse non-stationary bandit problem is similar to the one described above, with the difference that pre-determined segments are used in place of task boundaries, and we require the base algorithm to have a guarantee for a notion of \textit{dynamic regret}: for any $1\le i\le j\le N$, and letting $L=\sum_{n=i}^j \tau_n$,
\vspace{-0.2cm}
\begin{equation}
\label{eq:basedynamicregret}
\sup_{(r_n)_{n=i}^j} \EE{\sum_{n=i}^j \sum_{t=1}^{\tau_n} (\max_{a\in [K]} r_{n}(a) - r_{n}(A_{n,t}))} \le B_{L,j-i,K},
\end{equation}
where we naturally extend the upper-bound notation to indicate the number of task changes in the segment of length $L$, and typically $B_{L,j-i,K}=\widetilde O(\sqrt{L(j-i+1)K})$. An example of such a base algorithm, which does not need to know the task boundaries and lengths, is \AdS~\citep{ADSWITCH-auer19a}.

\subsection{Contributions}\label{sec:contribution}
In \cref{sec:unknown}, we present an algorithm for our sparse non-stationary bandit problem, 
and show that its dynamic regret scales as $\widetilde O(M {N}^{-1/3} T (\log K)^{1/3} + M \sqrt{M N T})$.
This algorithm is based on the aforementioned reduction to bandit subset selection problem and uses a bandit submodular optimization method, and needs to know the number of change points in advance.
Without any restrictions on the set of optimal arms, the optimal rate for the non-stationary problem is $\widetilde{O}(\sqrt{KNT})$~\citep{ADSWITCH-auer19a,CLLW-2019,WL-2021}.\footnote{This rate is achieved by algorithms such as \AdS of \citet{ADSWITCH-auer19a} without any prior knowledge of $T$ or $N$.} For small $N$, this baseline rate cannot be improved. %
Therefore, we are mainly interested in the regime of a large number of tasks and a small number of optimal arms, for which our regret upper bound is smaller than the baseline regret. 

The same reduction to submodular optimization also applies to the bandit meta-learning problem, and leads to a regret bound that is better than the simple baseline of $O(\sum_{n=1}^N B_{\tau_n,K})$; this is shown in \cref{sec:known}. 
Importantly, in this setting, our regret guarantees hold even in the more general adversarial problems where the reward vector can change within each task.

In Section~\ref{sec:greedy}, we analyze the bandit meta-learning problem in the realizable setting with stochastic tasks, and provide two algorithms which provide sample-efficient solutions to the problem under some assumptions on the identifiability of the optimal arms in each task. 
When all tasks have the same length $\tau$, our computationally efficient algorithm \greedy achieves an $O(N B_{\tau,M (1+\log N)}) + \widetilde O(N^{1/2})$ regret, paying a small $\log N$ factor in the regret for computational efficiency. To remove this extra factor we design \pmml, which achieves the desired $O(N B_{\tau,M})+\widetilde O(N^{1/2})$ regret, at the cost of a computational complexity that is potentially exponential in $M$.
Although \greedy is similar to the greedy solution in offline submodular maximization, the proof technique is quite different and exploits the special structure of the problem and results in an improved regret. A naive reduction to bandit submodular maximization would yield only an $\widetilde O(N B_{\tau,M})+\widetilde O(N^{2/3})$ regret.



\section{Reduction to subset-selection and bandit submodular maximization}
\label{sec:subset}

As explained in Section~\ref{sec:approach}, we reduce our problems to a bandit subset-selection problem. However, instead of learning the subset of the best arms task by task (whose boundaries are unknown in non-stationary problems), it will be convenient to divide the time horizon $T$ into $N'$ segments of equal length 
$\tau'=T/N'$ (in meta-learning problems when tasks are of equal length, we can choose $N'=N$ making segments and tasks coincide), and learn the optimal arms from segment to segment. Consider segment $n$, $[(n-1)\tau'+1, n\tau')$. Without loss of generality, we assume that a new task starts at the beginning of each segment (we can redefine the task boundaries accordingly), so we have at most $N+N'-1$ tasks. That is, denoting by $N_n$ the number of tasks in segment $n$, we have 
\begin{align}
    \label{eq:segnum}
    \sum_{n=1}^{N'} N_n  \le N+N'-1\; .
\end{align} 
We also denote $\tau_{n,u}$ and $r_{n,u}$ respectively the length and mean reward of $u$'th task in segment $n$.

In segment $n$, the learner chooses a subset of arms $S_n\in \cS=\{S:S\in 2^{[K]}, |S|\le M\}$ and runs a base bandit algorithm on that subset for $\tau'$ steps and receives a pseudo-reward\footnote{We call it pseudo-reward since it considers the mean reward functions not the actual random actions. 
}
\begin{align*}
\sum_{u=1}^{N_n}\sum_{t=1}^{\tau_{n,u}} r_{n,u}(A_{n,u,t})
&= \sum_{u=1}^{N_n}\bigg( \tau_{n,u} \max_{a\in S_n} r_{n,u}(a)
- \sum_{t=1}^{\tau_{n,u}}\left(\max_{a\in S_n} r_{n,u}(a) - r_{n,u}(A_{n,u,t}) \right)\bigg)
\\
&\doteq f_n(S_n) - \tau' \varepsilon_n\;,
\end{align*}
where $A_{n,u,t}$ is the learner's action in time step $t$ of task $u$ of segment $n$, $f_n(S) \doteq \sum_{u=1}^{N_n} \tau_{n,u} f_{n,u}(S)$ and $f_{n,u}(S)\doteq \underset{a\in S}{\max}~ r_{n,u}(a)$ is the max-reward function for a set of arms $S$ and reward function $r_{n,u}$, and $\varepsilon_n$ is the average ``noise'' per time step observed by the agent. We assume the base algorithm satisfies \eqref{eq:basedynamicregret},
$\tau' \E[\varepsilon_n] \le B_{\tau',N_n,M}$.
We prove in \cref{app:submod} that $f_n\in \cF$, the family of submodular functions, since it is an affine combination of finitely many submodular functions. Now we can bound the regret in the sparse non-stationary bandit problem as follows (proof in \cref{app:metalearning2subset}):
\begin{lemma}
\label{lemma:metalearning2subset}
For any policy running a base algorithm satisfying \eqref{eq:basedynamicregret} in each segment $n$ on a selected subset of arms $S_n$, we have
$
R_T 
\le~\!\! 
\underset{f_1,\ldots,f_{N'}{\in \cF}}{\sup}\!~ \underset{S\in \cS}{\max} \; \E\!\left[\sum_{n=1}^{N'} \!\Big(f_n(S)\! - \!f_n (S_{n})\! +\! B_{\tau',N_n,M} \Big)\! \right]\!\!.
$
\end{lemma}
Thus, the sparse non-stationary bandit problem can be reduced to minimizing a notion of regret where in segment $n$, the learner chooses a subset $S_n\in\cS$ and observes $f_n(S_n)-\tau'\varepsilon_n$. 
Since $f_n$ is submodular, this reduction allows us to leverage the literature on bandit submodular optimization to get a bound on $R_T$. %
\subsection{Bandit submodular maximization}
\label{sec:submodular-disc}

As mentioned above, the problem of subset selection %
is an instance of online submodular maximization. \citet{streeter2007online} studied the online submodular maximization problem in four different settings: the full-information setting where the function $f_n$ is fully observed at the end of round $n$; the priced feedback model where the learner can observe $f_n$ by paying a price and the price is added to the total regret; a partially transparent model where values of $f_n$ for some subsets are revealed, and the bandit setting where only $f_n(S_n)$ is observed. For the full-information and partially transparent models, an $O(\sqrt{N})$ regret is shown, while for the priced feedback and bandit model, an $O(N^{2/3})$ regret is shown. \citet{RKJ-2008} provide a similar algorithm to that of \citet{streeter2007online} for a particular ranking problem, with the more informative partially transparent feedback model, and also obtain an $O(N^{1/2})$ regret bound.
The priced feedback model is similar to problems where the best arms can be identified in every task, which we study in Section~\ref{sec:greedy}. 

\section{A general solution based on submodular maximization}
\label{sec:unknown}

In this section we present our first algorithm, \BOG, for ``online submodular bandit subset selection'', based on the above reduction and the general submodular maximization algorithm \OGO of \citet{streeter2007online}. The algorithm is applicable in the agnostic setting and its pseudo-code is given in \cref{alg:BanditOG}. \BOG applies $\Mlogn=\mppr$ expert algorithms (i.e, regret minimization algorithms in the full information setting) over the $K$ arms, denoted by $\mathcal{E}_1,\ldots,\mathcal{E}_{\Mlogn}$, where the role of $\mathcal{E}_i$ is to learn the $i$th ``best'' action.

In segment $n$, each expert picks an action. The algorithm \emph{exploits} (\ext) the set of $\Mlogn$ actions picked by the experts with probability $1-\gamma_n$, 
i.e, a base algorithm \base is executed on this set for $\tau'$ steps. With probability $\gamma_n$, the algorithm \emph{explores} (\exr), meaning that first a random index $i\in [\Mlogn]$ is chosen uniformly at random, and then the set of $i-1$ actions picked by the experts $\{\ca{E}_1,\cdots,\ca{E}_{i-1}\}$ is chosen, and together with a random action $a'_i$, \base is executed on this set of $i$ actions, $S_{n:i}$, for $\tau'$ steps.
When exploring, the expert whose action is replaced with a random action ($\mathcal{E}_i$) is updated with a reward function where the reward for the chosen action $a'_i$ is the average reward of \base in the segment (approximately $f_n(S_{n:i})/\tau'$ up to error $\varepsilon_n/\tau'$), while for all other actions the reward is zero, and all other experts are updated with an all-zero reward function.\footnote{This is simply to construct an unbiased estimator and use importance sampling. We provide no feedback to the experts during the exploitation phase. It is reasonable to expect that by using such feedback we can improve the empirical performance of the algorithm, but using the feedback is not going to improve the theoretical guarantees.}
In this way, $\mathcal{E}_1,\ldots,\mathcal{E}_i$ jointly learn the identity of the best $i$-set given the (approximate) reward function $\sum_{n=1}^N f_n$, hence approximating a greedy solution for finding the top $M$ arms (essentially, the ``real'' reward of expert $\mathcal{E}_i$ for action $a$ is $f_n(S_{n:i-1}\cup\{a\})-f_n(S_{n:i-1})$). \BOG should be viewed as a simulation of the off-line greedy procedure, which constructs its solution incrementally~\citep{streeter2007online}. When an index $i$ is chosen, the algorithm is learning the $i$th choice of the off-line greedy procedure and therefore only a subset of size $i$ is played.

Our requirement about the expert algorithm is that it achieves an $O(\sqrt{v \log(K)})$ regret over $v$ time steps relative to the best action selected in hindsight; this is achieved by all standard expert algorithms, such as exponential weights \citep{PLG}.
The choice of \base depends on which setting we solve.


\begin{algorithm}[tb]
\caption{\BOG: Online Submodular Bandit Subset Selection for Non-Stationary Bandits and Meta-Learning}
\label{alg:BanditOG}
\begin{algorithmic}[1]
\STATE {\bfseries Input}: Subset size $M$, segment length $\tau'$, {\tt Expert} algorithms $\mathcal{E}_1,\cdots,\mathcal{E}_{\Mlogn}$;
\FOR{$n \in [N']$}
    \STATE For each $i\in[\Mlogn]$, use $\mathcal{E}_i$ to choose an action $a_i$ 
    \STATE Set $S_{n}=\{a_1,\cdots,a_{\Mlogn}\}$
    \STATE With prob. $\gamma_n$, $E_{n} = \exr$, otherwise $E_{n} = \ext$
        \IF{$E_{n} = \ext$}
        \STATE Run \base on $S_{n}$ for $\tau'$ steps
        \ELSE
        \STATE Choose $i\in[\Mlogn]$ uniformly at random
        \STATE Choose a new action $a'_{i}$ uniformly at random 
        \STATE Replace $i$'th element of $S_{n}$ with $a'_{i}$: 
        \STATE \quad $S_{n:i}\gets\{a_1,\cdots,a_{i-1},a'_i\}$
        \STATE Run \base on $S_{n:i}$ for $\tau'$ steps
        \STATE Feed back the average reward over the segment as a reward to $\mathcal{E}_i$ for $a_i'$, and zero reward for all other actions and experts
        \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}



\subsection{The sparse non-stationary bandit setting}


To choose \base, notice that in the sparse non-stationary bandit problem, every segment may contain multiple tasks. Therefore, we need to choose an algorithm that is able to solve non-stationary bandit problems, without the knowledge change points. Hence, we use the \AdS algorithm of \citet{ADSWITCH-auer19a} as \base in \cref{alg:BanditOG}, giving $B_{\tau',N_n,\Mlogn}=\sqrt{\Mlogn N_n \tau'}$ for segment $n$ in Lemma~\ref{lemma:metalearning2subset}. 
The performance of the algorithm is analyzed in the next theorem (proved in \cref{sec:BOGpfs}).
Note that the algorithm does not need to know when the tasks change and the tasks can be of different lengths.
\jtodo{how to use unknown N results}
\begin{restatable}[]{theoremi}{BOGNonStatOpt}
\label{thm:BOG-NonStat-Opt}
The regret of \BOG using \AdS as \base, with $N'$ segments each of size $\tau'=T/N'$, and using exploration probability $\gamma_n=\gammaOne
$ is $R_T = \tilde O(
T {N'}^{-1/3} (\Mlogn^4 K \log K)^{1/3} + \Mlogn \sqrt{\Mlogn N' T} )$. 

\end{restatable}
We are mainly interested in the regime of large number of switches and small number of optimal arms. 
If $N \ge \Nthresh$ and $M \le K^{1/3}$, with the choice of $N'=N$, we have 
$\Mlogn (\log K)^{1/3} N^{-1/3} T \le \Mlogn^{3/2}\sqrt{N T}$, and the regret of \BOG improves upon the $\tilde{O}(\sqrt{KTN})$ bound of standard non-stationary bandit algorithms (such as \AdS).
In the case of a small number of switches, however, the simple baseline of $\tilde{O}(\sqrt{KTN})$ can be smaller than our bound, and the learner should simply play a standard non-stationary bandit algorithm. %
At the extreme that $N=O(1)$, i.e. only a few changes in the environment, the regret bound $\tilde{O}(\sqrt{KNT})$ cannot be improved. On the other hand, when $N$ is large compared to $T$, it is easy to establish a $O(\sqrt{MNT})$ lower bound, and therefore our $\tilde{O}(M\sqrt{MNT})$ bound is optimal up to a factor of $M$. Closing this gap remains an open question. We can improve the bounds in certain regimes by further tuning of the parameters, which is discussed in more details in \cref{sec:BOGpfs}.

The algorithm needs to know the number of changes $N$ in advance: the segment length $\tau'$ depends on $N'$, and as the proof of \cref{thm:BOG-NonStat-Opt} reveals, we need $N'\ge N$ to have the above regret upper bound. In the next section, we consider a meta-learning setting where segment lengths are fixed in advance. In that case, we can have a version of the algorithm that does not need to have $N$ as input.  


\subsection{Bandit meta-learning}\label{sec:known}

In this section we consider the bandit meta-learning problem with tasks of equal and known length $\tau$. Again, we apply \BOG, instantiated now with different parameters and a different \base algorithm. Since we know $\tau$, we can always introduce a segmentation such that each segment contains a single task only (possibly only a part of a task), and choose \base to be an algorithm designed for a multi-armed bandit problem such as the well-known \UCB algorithm \citep{ACFS-2002} when tasks are stochastic bandits, or EXP3 algorithm \citep{ACFS-1995} when tasks are adversarial bandits. 

\begin{restatable}{corollaryi}{thmBG}
\label{thm:BOG}
Consider \BOG with \UCB as \base in a meta-learning problem with $N$ stochastic bandit tasks of equal length $\tau$. %
By the choice of $\tau'=\tau$ and $\gamma_n=\gammaOnenprime$, the regret is $R_T = \tilde O(
\tau {N}^{2/3} (\Mlogn^4 K \log K)^{1/3}
+\Mlogn N\sqrt{\Mlogn \tau})$. 
\end{restatable}
The proof is omitted as it follows the proof argument of \cref{thm:BOG-NonStat-Opt}. Again, in the regime of large number of tasks and small number of optimal arms, our bound improves upon the $\tilde{O}(N\sqrt{K\tau})$ bound of the trivial solution of running an independent UCB algorithm in each task.

We can extend the above result to an adversarial setting, where the reward vector can change in every time step, by using an EXP3 algorithm instead of UCB. Such an extension is  not possible in the sparse non-stationary setting as currently we are not aware of a base algorithm with \textit{adaptive} dynamic regret guarantee in the adversarial setting.




\begin{remarki}[Variable task lengths]
Consider problems with non-equal task lengths where the learner only gets to know the length of each task when they begin. To deal with this situation, we construct an exponential grid for the task lengths with $b:=\log(\max_n\tau_n)\leq \log T$ buckets where bucket $i$ is $[\underbar{$\tau$}_i:=2^{i-1}, \overline{\tau}_i:=2^i]$. %
Now we run a copy of \BOG on the tasks falling in each bucket as they arrive. Let $N^{(i)}$ denote the number of tasks that fall in bucket $i$. Then by \cref{thm:BOG}, the total regret satisfies
$%
    R_T\leq \sum_{i=1}^{b}\tilde{O}(
    \Mlogn^{4/3} (N^{(i)})^{2/3}K^{1/3}\overline{\tau}_i
    +N^{(i)} \Mlogn^{3/2}\sqrt{\overline{\tau}_i}).~ 
$%
\end{remarki}


\section{Bandit meta-learning under an identifiability condition}
\label{sec:greedy}

In this section, we study the bandit meta-learning problem in the \emph{realizable} setting under the assumption that the learner has access to an exploration method that reveals optimal actions. We further assume that the tasks are of equal length $\tau$.

\begin{assumptioni}[Efficient Identification]
\label{assumption:identification}
There exists a set of $M$ arms that has a non-empty intersection with the set of optimal arms in each task. Also, the learner has access to a best-arm-identification (BAI) procedure that for some $\delta \in [0,1]$, with probability at least $1-\delta/N$, identifies the set of optimal arms if executed in a task (for at most $\tau$ steps)\footnote{Note that the Efficient Identification assumption requires the BAI procedure to return only optimal arms. This choice is for simplicity and could easily be relaxed to allow the returned set to be all arms with sub-optimality gap smaller than $\Theta(\sqrt{M\log (N/\delta)/\tau})$; we discuss this in more details in the analysis.}.
\end{assumptioni}
The Efficient Identification assumption is a special case of the priced feedback model of \citet{streeter2007online}. 
If for any task $n$ with optimal arms $S^*_n \subset [K]$, we have $r_n(a^*_n) - \max_{a\not\in S^*_n}r_n(a) \ge \Delta$ for all $a^*_n \in S^*_n$ (note that $r_n(a^*_n)$ is the same for all $a^*_n\in S^*_n$) for some $\Delta=\Theta(\sqrt{K\log (N/\delta)/\tau})$, a properly tuned \emph{phased elimination} (PE)\footnote{Improved \UCB of \citet{AO-2010} runs exponentially growing phases and maintains an active set of arms with gaps twice smaller in every step.} procedure~\citep{AO-2010} returns the set of optimal arms with probability at least $1-\delta/N$. 
The cumulative worst-case regret of PE in a task with $K$ arms is $B'_{\tau,K}=\Theta(B_{\tau,K})$ \citep{AO-2010}, see 
\citet{lattimore-Bandit} for details. With a slight abuse of notation, in this section we use $B_{\tau,K}$ to denote $\max\{B_{\tau,K},B'_{\tau,K}\}$.

Akin to \BOG, we disentangle exploration (\exr) and exploitation (\ext) at a meta-level.
In \exr mode, the learner executes a BAI on all arms, and (by Assumption~\ref{assumption:identification}) observes, with high probability, the set of optimal actions, $S_n^*$. 
The price of this information is a large regret denoted by $\Cinfo$, which for a properly tuned PE, we know $\Cinfo=B_{\tau,K}>B'_{\tau,M}$.
So, since we aim for $\reg_T \le \widetilde O(N B_{\tau,M}) + o(N)$, we should keep the number of \exr~calls small. In \ext mode, the learner executes a base bandit algorithm on a chosen subset $S_n$, constructed using the previously identified optimal actions $\cI_n=\bigcup_{j<n: E_j=\exr} \{S^*_j\}$.


Let $s_n$ be the size of $S_n$. If $S_n\cap S_n^*\neq \emptyset$, the regret of the base algorithm is bounded by $\Cgood=B_{\tau,s_n}$. Otherwise, since the performance gap between the optimal arms and the arms in $S_n$ can be arbitrary, the regret in the task can be as large as $\Cbad=\tau$. Note that to keep $\Cgood$ small, the subset $S_n$ should be as small as possible. Ideally, $S_n$ should be a subset of size $M$ that has non-empty overlap with all members of $\cI_n$. However, the problem of finding such $S_n$ 
is the so-called \emph{hitting set} problem, which is known to be NP-Complete \citep{feige2004approximating}.

A simple greedy algorithm can be used to get an approximate solution efficiently (see, e.g, \citealp{streeter2007online}):\todoa{Explain what the greedy algorithm does} it has polynomial computation complexity and 
it finds a subset of size at most $M(1+\log N)$ that contains an optimal action for each task. We say an action $a\in [K]$ covers task $j$ if $a\in S_j^*$. The greedy method, denoted by \textsc{Greedy}, starts with an empty set and at each stage, it adds the action that covers the largest number of uncovered tasks in $\cI_n$, until all tasks are covered.

We also propose \pmml, that is based on an elimination procedure; 
the learner maintains an active set of possible $M$-subsets compatible with the \exr history, and all subsets that are inconsistent with $\cI_n$ are eliminated. In $\ext$ mode, a subset is selected uniformly at random from the set of active subsets. As we will show, this algorithm improves the regret by a factor of $\log N$, although it is not computationally efficient.


\begin{algorithm}[tb]
 \caption{\bass: Bandit Subset Selection for Meta-Learning} \label{alg:ossem}
 \begin{algorithmic}[1]
\STATE {\bfseries Option:} Greedy \greedy~{(G)}, Elimination-based \pmml~{(E)}\;

\STATE {\bfseries Input:} \base (efficient $K$-armed bandit algorithm), best arm identification algorithm \texttt{BAI}, \exr~probabilities $p_n$, (E) subset size $M$\;

\STATE  \textbf{Initialize:} Let
 {(G)} ${\cI_0}=\emptyset$; {(E)} $\cX_0$ be the set of all $M$-subsets of $[K]$.\;
 \FOR{$n=1,2,\dots,N$}{
  
\STATE  With prob. $p_n$, let $E_n=\textsc{Exr}$; otherwise $E_n=\textsc{Ext}$\;
  \IF{$E_n=\textsc{Exr}$ or $n=1$}{
  
\STATE  Run \texttt{BAI} on all arms and observe the best arms $S^*_n$ of this task\;
  
\STATE  {(G)} Update $\cI_n = \cI_{n-1} \cup \{S^*_n\}$\;

\STATE  {(E)} Let $\cX_n=\{S \in \cX_{n-1}: S\cap S^*_n \neq \emptyset\}$ be elements of $\cX_{n-1}$ with non-empty overlap with $S^*_n$; 
  }\ELSE{
  
\STATE  {(G)} Find $S_n$ by \textsc{Greedy} s.t. $\forall S\in\cI_n, S_n\cap S \neq \emptyset$\;
  
\STATE  {(E)} Sample $S_n$ uniformly at random from $\cX_n$\;
 
\STATE Run \base algorithm on $S_n$ \;
  }\ENDIF
 }\ENDFOR
\end{algorithmic}
\end{algorithm}

The analysis of \greedy depends on the \emph{cost-to-go} function of the following game between the learner and environment. At round $n$, the learner may choose $E_n\in\{\exr,\ext\}$ with distribution $p_n=P(E_n=\exr)$ and cost $\Cinfo$. The environment may choose a best arm $a^*_n$ that the learner already knows about which costs $\Cgood$ (i.e, $a^*_n \in S_n$
) or choose an optimal arm set $S_n^*$ so that $S_n^*\cap S_n=\emptyset$, with cost $\Cbad$. Let $q_n=P(S_n^*\cap S_n=\emptyset)$.
The regret of \greedy is bounded by the cost of the learner in this simple game, if we assume  $\delta=0$ in \cref{assumption:identification}.
The learner is a (randomized) function of 
$\cI$, hence we can easily define and write the minimax cost-to-go function as 
\begin{align}
\begin{split}
    V_N(\cI)  &= 0~~\text{and for } n<N, 
    \\
     V_n(\cI) 
     &= \min_{p}\max_{q} \{ p \Cinfo + q(1-p)\Cbad 
     +(1-q)(1-p)\Cgood 
     \\&\qquad
      +(1-pq)V_{n+1}(\cI) 
     +pq V_{n+1}(\cI\cup \{S_n^*\}) \}.  \label{eq:cost-to-go-def}
\end{split}
\end{align}
For the last equality note that when the environment reveals a new action (happens with probability $q$) and the learner explores (with probability $p$), its current knowledge set $\cI$ is incremented.
The optimal cost-to-go function $V_n$ above corresponds to the case of $\delta=0$ in Assumption~\ref{assumption:identification}, and $V_0(\emptyset)$ gives the minimax regret for the family of algorithms with the limited choice described.
Therefore, when the BAI algorithm is successful, almost surely, $\reg_T \le V_0(\emptyset)$. For $\delta>0$, using a union bound, we can show
$\reg_T \le V_0(\emptyset) + \delta N\tau$. 
Setting $\delta=1/(N\tau)$ ensures that $\delta N\tau$ is negligible. 
Finally, if the BAI algorithm only returns a set of approximately optimal arms satisfying $r_n(a) \ge r_n(a^*_n)-\Delta$ for all arms $a$ selected, the meta-regret can be bounded trivially as 
$\reg_T \le V_0(\emptyset) + (\delta + \Delta)N\tau$.

Before deriving $V_0(\emptyset)$ in the general case, we consider the more restricted setting where each task has a unique optimum.

\paragraph{Characterizing an optimal policy in the case of unique optimal arms:}
Assume there is a unique and identifiable optimal arm in each task. 
\begin{assumptioni}[Unique Identification]
\label{assumption:unique-identification}
Assumption~\ref{assumption:identification} holds, and each task has a unique best arm.
\end{assumptioni}

\begin{theoremi}
\label{thm:unique-identification}
In the simple game, 
\[
V_0(\emptyset) \le N B_{\tau,M} + M \sqrt{2(\Cinfo - \Cgood)(\Cbad - \Cgood) N}\;.
\]
Therefore, under \cref{assumption:unique-identification}, the regret of \greedy can be bounded, for an appropriate selection of the parameters
$p_n=\Theta(1/\sqrt{N-n})$, as
\[
\reg_T  \le N B_{\tau,M} + M \sqrt{B_{\tau,K} N\tau} + \delta N\tau\;.
\]
\end{theoremi}

We prove this in \cref{sec:thm:unique-identification-pf} by solving the min-max problem in \eqref{eq:cost-to-go-def} for $V_n$.
Interestingly, the exploration probability $p_n$ increases as $\Theta(1/\sqrt{N-n})$. This might seem counter-intuitive at first as typically the exploration rate decreases in most online learning algorithms. The intuition is that as $n$ gets closer to $N$, if $s<M$, the adversary does not have much time left to use the remaining budget to make the learner suffer a big cost. Therefore, the adversary needs to increase its probability of choosing a new optimal arm.



\paragraph{The more general case:}
Now we consider the more general case with potentially multiple optimal arms in each task. 
\begin{theoremi}
\label{thm:greedy}
Let $M'=M(1+\log N)$. 
Under \cref{assumption:identification}, the regret of the \greedy~algorithm with exploration probability $p_n=\sqrt{\frac{|S_n| K \tau}{N B_{\tau,K}}}$ for all $n$ is bounded as
\begin{align*}
\reg_T \le N B_{\tau,M'} + M B_{\tau,K} +\sqrt{M K B_{\tau,K} N \tau} + \delta N\tau \;.
\end{align*}
\end{theoremi}
The proof is similar in spirit to that of Theorem~\ref{thm:unique-identification} and is deferred to Appendix~\ref{ap:proof-thm-greedy}. The regret guarantee holds in the realizable setting, but the \greedy~algorithm does not need $M$ as input. The next theorem shows that the regret of \pmml~is bounded as $N B_{\tau,M} + o(N)$, which is smaller than the regret of the \greedy~ algorithm by a factor of $\log N$; note, however, that \pmml is not computationally efficient and also requires $M$ as input. The proof of the theorem is in Appendix~\ref{app:partial-monitoring}.
\begin{theoremi}
\label{thm:PM}
Under \cref{assumption:identification}, with constant exploration probability $p_n=\left(\frac{\tau}{K}\right)^{1/4}\sqrt{\frac{\log K}{N}}$, the regret of the \pmml~ algorithm is bounded as $\reg_T \le N B_{\tau,M} + O(\tau^{3/4}K^{1/4}\sqrt{N M \log K})$.
\end{theoremi}

\begin{remarki}[Connections with partial monitoring games]
The setting of this section can be viewed more generally as a partial monitoring game. Partial monitoring is a general framework in online learning that disentangles rewards and observations (information). 
In our bandit meta-learning problem, different actions of the meta-learner (\textsc{Exr} and \textsc{Ext}) provide different levels of information and have different costs, and the problem can be reduced to a partial monitoring game on $\cX$, the set of $M$-subsets of $[K]$. More details are in Appendix~\ref{app:partial-monitoring}.
\end{remarki}

\section{Related work}
\label{sec:related}

Our bandit solution is based on subset selection, which connects it to many branches of online learning and bandit literature. %

\noindent\textbf{Non-stationary experts/bandits with long-term memory. } The sparse non-stationary bandit problem is the bandit variant of experts problem with small set of optimal arms whose study goes back to \citet{Bousquet-Warmuth-2002}. %
The only result in the bandit setting that we are aware of is the work of \citet{ZLDW-2019}, who show an algorithm for competing against a small set of optimal arms in an adversarial setting with sparse reward vectors. The solution of \citet{ZLDW-2019} has similarities with our approach, as both solutions are reduction-based and employ a meta-learner that plays with base algorithms. Similar to our approach, the meta-learner of \citet{ZLDW-2019} needs to satisfy a static regret guarantee, while the base algorithm needs to satisfy a dynamic regret guarantee. The algorithm of \citet{ZLDW-2019} also requires the number of change points as input and its dynamic regret is
$%
\Tilde O ((s N)^{1/3} (MT)^{2/3} + M \sqrt{s T \log K} + M K^3 \log T) \,,~
$%
where $s=\max_n \|r_n\|_0$ is the number of non-zero elements in reward vectors. Notice that without this sparsity condition, the above dynamic regret is worse than $\Tilde O(\sqrt{KNT})$ regret of EXP3.S. When $s$ is a small constant, the above bound improves upon the regret of EXP3.S when $M^{4/3}(T/N)^{1/3} < K < (TN/M^2)^{1/5}$.

\noindent\textbf{Meta-learning in adversarial bandits.} \citet{balcan2022meta} studies bandit meta-learning problems with adversarial bandit tasks. They introduce a meta-learning algorithm that tunes the initialization and step-size of the online mirror decent base algorithm. \citet{balcan2022meta} show that their algorithm achieves  $\min_{\beta\in(0,1]}\tilde{O}(N\sqrt{H_\beta K^\beta \tau/\beta}+N^{1-\beta/6})$ total regret, where $H_\beta$ is a notion of entropy. When a subset of size $M$ contains the optimal arms of most tasks, then by the choice of $\beta=1/\log(K)$ the regret bound simplifies to $\tilde{O}(N\sqrt{M\tau} + N^{1-1/(6\log K)})$.  
Compared to our results in Section~\ref{sec:known}, their convergence rate of $\tilde{O}(1/N^{1/(6\log K)})$ is much slower than our convergence rate of $\tilde{O}(1/N^{1/3})$. However, their task-averaged regret is $O(\sqrt{M \tau})$, whereas it is $O(M\sqrt{M \tau})$ in our case. Finally, the regret bound of \citet{balcan2022meta} adaptively holds for the best value of $M$, while $M$ is an input to our algorithm.
\citet{osadchiy2022online} further improves the results of \citet{balcan2022meta} under extra identifiability assumptions.  

\noindent\textbf{Slate bandits. } The reduction in Section~\ref{sec:subset} is an instance of slate bandit problems with a non-separable cost function~\citep{DVJ-2019,RAZK-2020,KRS-2010}.
\citet{RAZK-2020} study the problem in the stochastic setting, where the reward parameter is fixed throughout the game. \citet{MM-2019} study a problem that includes the probabilistic maximum coverage as a special case. They obtain problem-dependent logarithmic and problem-independent $O(\sqrt{N})$ regret bounds. However, the feedback structure in this work is richer than our setting. Applied to our problem, they assume that in each round, for each item and task pair, a random variable is observed whose expected value is the probability that the item is the optimal arm in that task.


\noindent\textbf{Meta-learning and bandit meta-learning. }
Meta, Multi-Task, and Transfer Learning \citep{baxter2000model,caruana1997multitask,thrun1996learning} are related machine learning problems concerned with learning a lower dimensional subspace across tasks. In that sense, our work is connected to other theoretical studies \citep{franceschi2018bilevel,denevi2018incremental,DCSP-2018,DCGP-2019,KSSKO-2020,khodak2019provable,TJJ-2021} though indeed we focus on the bandit learning setting. Various other ways of modelling structure have been proposed and studied in bandit meta-learning. A special case of our problem was studied by \citet{ALM-2013} where $K$-armed bandit problems are sampled from a prior over a finite set of tasks. \citet{PSJO-2021} consider a continual learning setting where  the bandit environment changes under a Lipschitz condition. \citet{kveton-2020} observe that the hyperparameters of bandit algorithms can be learned by gradient descent across tasks. Learning regularization for bandit algorithms \citep{KKZHMBS-2021,CLP-2020} are also proposed, building on the biased regularization ideas from \citet{baxter2000model}. Interestingly, these contextual problems are also connected with latent and clustering of bandit models \citep{MM-2014,GLZ-2014,HKZCAB-2020,HKZCAGB-2020}.

\noindent\textbf{Bandits with very large action spaces. } 
As $K$ grows very large, our bandit meta-learning problem is akin to infinitely many armed bandits \citep{BCZHS-1997,WAM-2008,BP-2013,CV-2015,chan2020infinite} and countable-armed bandits~\citep{Kalvit-Zeevi-2020} though these settings do not have a meta-learning aspect. 

\section{Experiments}

In this section, we study the performance of our algorithms on synthetic environments. 
The experiments include: 1) \greedy
~\footnote{\pmml~is computationally too expensive so we only run it on smaller settings in \cref{sec:FurtherExperiments}.}
from \cref{sec:greedy}, 2) \cref{alg:BanditOG}, \BOG, 3) \MOSS which is agnostic MOSS \citep{AB-2009} running independently on the tasks without any knowledge of the optimal $M$-subset, 4) \OptMoss, an oracle MOSS that plays only the arms in the optimal $M$-subset, and its performance constitutes an empirical lower bound on the achievable regret, and 5) \OGO, which is \BOG with the choice of $\tau'=\tau$ and optimized $\gamma$. Error bars are $\pm1$ standard deviation computed over $5$ independent runs.

We study the impact of four variables on the regret: number of tasks $N$, length of each task $\tau$, number of arms in each task $K$, and the optimal subset size $M$. To do so, we fix a default setting of $(N,\tau,K,M)$ and for each experiment we let one of these parameters vary. The problems are generated by an \emph{oblivious} adversary (see \cref{sec:FurtherExperiments} for further details). 

\cref{fig:all} demonstrates the impact of $N$ and $M$. Further experiments in \cref{sec:FurtherExperiments} illustrate the effect of all four variables including $\tau$ and $K$. 
Under \cref{assumption:identification} (left two plots), \greedy~outperforms all methods with a regret close to that of the oracle \OptMoss. When this assumption does not hold (right two plots), \BOG outperforms the other algorithms, while \greedy naturally has high variance.

\begin{figure*}[htb!]
    \centering
    \begin{minipage}{.24\textwidth}
        \includegraphics[width=\textwidth]{img/Adversarial_task_exp.png}
    \end{minipage}
    \begin{minipage}{.24\textwidth}
        \includegraphics[width=\textwidth]{img/Adversarial_subset_exp.png}
    \end{minipage}
    \begin{minipage}{.24\textwidth}
        \includegraphics[width=\textwidth]{img/no_gap_small_tau_Adversarial_task_exp.png}
    \end{minipage}
    \begin{minipage}{.24\textwidth}
        \includegraphics[width=\textwidth]{img/no_gap_small_tau_Adversarial_subset_exp.png}
    \end{minipage}
        \includegraphics[width=\textwidth]{img/legend5.png}
    \vspace{-0.8cm}
    \caption{
    Default setting: $\setupOne$.
    In the right two plots $\tau=450$.
    Left to Right: Regret as a function of $N$ and $M$ under \cref{assumption:identification}. Regret as a function of $N$ and $M$ without \cref{assumption:identification}.
    }
    \label{fig:all}
\end{figure*}

\section{Discussion and Future Work}\label{sec:conclude}
We analyze a problem of $N$ tasks of $K$-armed bandits arriving sequentially, where the adversary is constrained to choose the optimal arm of each task in a smaller subset of $M$ arms. We consider two settings: bandit meta-learning and non-stationary bandits. We design an algorithm based on a reduction to bandit submodular optimization, and prove that its regret is $\tilde{O}(M N^{-1/3}T (\log K)^{1/3} + M^{3/2} \sqrt{N T})$. Under additional identifiability assumptions, we develop a meta-learning algorithm with an improved regret.

For the general non-stationary setting, we assume $N$ is known. Relaxing this assumption adaptively is left for further work. %


==> m small 10-18-2022_arXiv/macros.tex <==




\newcommand{\ca}[1]{\mathcal{#1}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\EE}[1]{\E\left[#1\right]}
\newcommand{\mP}{\mathbf{P}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\reg}{R}
\newcommand{\regm}{R^{\text{meta}}}
\newcommand{\base}{\ensuremath{\tt Base}\xspace}

\newcommand{\exr}{\textsc{Exr}\xspace}
\newcommand{\ext}{\textsc{Ext}\xspace}
\newcommand{\Cinfo}{\textbf{C}_{\texttt{info}}}
\newcommand{\Cgood}{\textbf{C}_{\texttt{hit}}}
\newcommand{\Cbad}{\textbf{C}_{\texttt{miss}}}

\newcommand{\Mlogn}{\tilde{M}}
\newcommand{\mpr}{\lceil M\log N\rceil}
\newcommand{\mppr}{\lceil M\log N'\rceil}





\newcommand{\AdS}{\ensuremath{\tt AdSwitch}\xspace}
\newcommand{\BOG}{\texttt{OS-BASS}\xspace} %
\newcommand{\OptMoss}{\texttt{Opt-MOSS}\xspace}
\newcommand{\OGO}{${\tt OG^o}$\xspace}
\newcommand{\OG}{\texttt{OG}\xspace}
\newcommand{\UCB}{{\tt UCB}\xspace}
\newcommand{\MOSS}{{\tt MOSS}\xspace}
\newcommand{\pmml}{\texttt{E-BASS}\xspace}
\newcommand{\greedy}{\texttt{G-BASS}\xspace}
\newcommand{\bass}{\texttt{BASS}\xspace}

\newcommand{\expSet}{X}
\newcommand{\optSets}{\I}
\newcommand{\rbar}{\bar{R}}
\newcommand{\tildelt}{\tilde{\Delta}}
\newcommand{\Rsm}{R_{\text{S}}}
\newcommand{\Rcov}{R_{\text{coverage}}}


\newcommand{\gd}{\text{GOOD}\xspace}
\newcommand{\bd}{\text{BAD}\xspace}
\newcommand{\out}{\text{OUT}\xspace}
\newcommand{\fmax}{f}
\newcommand{\wt}{w} %

\newcommand{\C}{\mathbf{C}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\T}{^\top}
\newcommand{\La}{\Lambda}
\newcommand{\lgk}{\log K}
\newcommand{\prob}[1]{\Pr(#1)}
\newcommand{\expp}[1]{\exp\left(#1\right)}
\newcommand{\dmin}{\Delta_{\min}}
\newcommand{\dmint}{\Delta_{\min,t}}
\newcommand{\muh}{\hat{\mu}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\sing}{\varsigma^2_{\max}}
\newcommand{\tethat}{\hat{\theta}}
\newcommand{\meanf}{f}
\newcommand{\cmin}{c_{\min}}
\newcommand{\Htwo}{H_{2,\text{lin}}}
\newcommand{\Nexp}{N_{\text{exp}}}
\usepackage{upgreek}

\newcommand{\gammaOne}{ \left(\frac{\Mlogn K\log K}{N'}\right)^{1/3}}
\newcommand{\gammaOneprime}{\left(\frac{\log K}{N'}\right)^{1/3}}
\newcommand{\gammaOnen}{\left(\frac{\Mlogn K\log K}{n}\right)^{1/3}}
\newcommand{\gammaOnenprime}{\left(\frac{\Mlogn K\log K}{n}\right)^{1/3}}
\newcommand{\gammaStar}{\frac{\sqrt{3\log K}M^{3/10}}{2 K^{6/5}(N\tau)^{3/10}}}
\newcommand{\tauThreshold}{\frac{\Mlogn N^{2/3}}{(\log K)^{2/3}}}
\newcommand{\uOne}{\frac{T^{3/5}\Mlogn^{12/5}}{K(\log K)^{3/5}}}
\newcommand{\tauChoice}{\frac{\Mlogn^{3/5} T^{2/5}}{(\log K)^{2/5}}}
\newcommand{\Rone}{R_1:=\Tilde{O}\left(\Mlogn(\frac{K}{N})^{1/3}T+M^{3/2}\sqrt{NT}\right)}
\newcommand{\uTwo}{\frac{T^{3/10}M^{6/5}}{K^{3/10}}}
\newcommand{\Nthresh}{\frac{T^{3/5} (\log K)^{2/5}}{\Mlogn^{3/5}}}
\newcommand{\tauThresholdMeta}{\frac{T^{2/5} K (\log K)^{3/5}}{\Mlogn^{12/5}}}

\newcommand{\NoGap}{where \cref{assumption:identification} is almost satisfied (only the minimum gap condition violated, large task length)}
\newcommand{\NoGapSmallt}{without \cref{assumption:identification} (no minimum gap and small task length)}


\usepackage{xcolor}
\renewcommand\thefootnote{\textcolor{red}{\arabic{footnote}}}

\newcommand{\setupOne}{(N,\tau,K,M)=(500,4500,30,10)\xspace}
\newcommand{\setupTwo}{(N,\tau,K,M)=(500,450,30,10)\xspace}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\usepackage[textsize=tiny, disable]{todonotes}

\PassOptionsToPackage{usenames,dvipsnames}{xcolor}

\newcommand{\todoy}[2][]{\xspace\todo[size=\scriptsize,color=red!20!white,#1]{Yasin: #2}\xspace}
\newcommand{\todoth}[2][]{\xspace\todo[size=\scriptsize,color=yellow!20!white,#1]{Thang: #2}\xspace}
\newcommand{\claire}[2][]{\xspace\todo[size=\scriptsize,color=blue!20!white,#1]{Claire: #2}\xspace}
\newcommand{\todoa}[2][]{\xspace\todo[size=\scriptsize,color=green!20!white,#1]{A: #2}\xspace}
\newcommand{\jtodo}[2][]{\xspace\todo[color=blue!5,size=\scriptsize,#1]{J: #2}\xspace}
\newcommand{\todomgh}[2][]{\xspace\todo[color=green!20,size=\scriptsize,#1]{MGH: #2}\xspace}

==> m small 10-18-2022_arXiv/preamble.tex <==
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} %
\usepackage{fullpage}

\usepackage[bookmarksopen=true,bookmarks=true,hidelinks,colorlinks=true,citecolor={blue}]{hyperref}
\usepackage{bookmark}


\newcommand{\theHalgorithm}{\arabic{algorithm}}

\usepackage{algorithm}
\usepackage{algorithmic}



\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

\usepackage[capitalize]{cleveref}

\usepackage{xspace}
\usepackage{thmtools} 
\usepackage{thm-restate}
 
\allowdisplaybreaks


\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{fact}[theorem]{Fact}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\newtheorem{theoremi}{Theorem}[section]
\newtheorem{propositioni}[theoremi]{Proposition}
\newtheorem{lemmai}[theorem]{Lemma}
\newtheorem{corollaryi}[theoremi]{Corollary}
\newtheorem{definitioni}[theoremi]{Definition}
\newtheorem{assumptioni}[theoremi]{Assumption}
\newtheorem{remarki}[theoremi]{Remark}

\usepackage[round,sectionbib]{natbib}
\bibliographystyle{plainnat}




